Computationally-Efficient Climate Predictions using Multi-Fidelity Surrogate Modelling

Accurately modelling the Earth's climate has widespread applications ranging from forecasting local weather to understanding global climate change. Low-fidelity simulations of climate phenomena are readily available, but high-fidelity simulations are expensive to obtain. We therefore investigate the potential of Gaussian process-based multi-fidelity surrogate modelling as a way to produce high-fidelity climate predictions at low cost. Specifically, our model combines the predictions of a low-fidelity Global Climate Model (GCM) and those of a high-fidelity Regional Climate Model (RCM) to produce high-fidelity temperature predictions for a mountainous region on the coastline of Peru. We are able to produce high-fidelity temperature predictions at significantly lower computational cost compared to the high-fidelity model alone: our predictions have an average error of $15.62^\circ\text{C}^2$ yet our approach only evaluates the high-fidelity model on 6% of the region of interest.

==> Figures/points/perf_sum_single.tex <==
\begin{tabular}{llrr}
\toprule
\multicolumn{2}{c}{Configuration} & \multicolumn{2}{c}{MSE} \\
            Model & Acquisition &  $\mu$ &  $\sigma$ \\
            % Model & Acquisition Function &  MSE Mean &  MSE Std \\
\midrule
               HF &          $a_{IVR,x}$ &     6.633 &   13.679 \\
               HF &           $a_{MV,x}$ &    10.159 &   25.286 \\
               HF &       $a_{Random,x}$ &    42.977 &   59.013 \\
\textbf{LF$\mathbf{\rightarrow}$HF} &          $\mathbf{a_{IVR,x}}$ &     \textbf{2.695} &    \textbf{1.550} \\
LF$\rightarrow$HF &           $a_{MV,x}$ &    16.212 &   40.716 \\
LF$\rightarrow$HF &       $a_{Random,x}$ &    42.876 &   58.378 \\
               MF &          $a_{IVR,x}$ &     7.723 &    6.656 \\
               MF &           $a_{MV,x}$ &    12.737 &   39.825 \\
               MF &       $a_{Random,x}$ &    13.658 &   16.553 \\
\bottomrule
\end{tabular}


==> Figures/squares/perf_best.tex <==
\begin{tabular}{lllrr}
\toprule
\multicolumn{3}{c}{Configuration} & \multicolumn{2}{c}{MSE} \\
            Model & Acquisition &  Grid Size &  $\mu$ &  $\sigma$ \\
\midrule
               MF &     $a_{IVR,B,\max}$ & Large Grid &    52.450 &   58.641 \\
               MF &    $a_{MV,B,\Sigma}$ & Small Grid &    19.907 &   21.226 \\
                \textbf{MF} &     \textbf{$a_{IVR,B,\max}$} & \textbf{Small Grid} &    \textbf{15.621} &   \textbf{18.109} \\
\bottomrule
\end{tabular}


==> Figures/squares/perf_sum.tex <==
\begin{tabular}{lllrr}
\toprule
\multicolumn{3}{c}{Configuration} & \multicolumn{2}{c}{MSE} \\
            Model & Acquisition &  Region Size &  $\mu$ &  $\sigma$ \\
\midrule
          HF &     $a_{IVR,B,\max}$ & Small &   115.863 &   30.295 \\
          HF &     $a_{IVR,B,\max}$ & Large &   138.184 &   25.079 \\
          HF &    $a_{MV,B,\Sigma}$ & Small &   167.076 &   25.116 \\
          HF &    $a_{MV,B,\Sigma}$ & Large &   170.951 &   27.235 \\
LF$\rightarrow$HF &     $a_{IVR,B,\max}$ & Small &    94.302 &   53.988 \\
LF$\rightarrow$HF &     $a_{IVR,B,\max}$ & Large &   140.887 &   50.381 \\
LF$\rightarrow$HF &    $a_{MV,B,\Sigma}$ & Small &   139.977 &   38.321 \\
LF$\rightarrow$HF &    $a_{MV,B,\Sigma}$ & Large &   144.278 &   47.940 \\
               \textbf{MF} &     \textbf{$a_{IVR,B,\max}$} & \textbf{Small} &    \textbf{15.621} &   \textbf{18.109} \\
               MF &     $a_{IVR,B,\max}$ & Large &    52.450 &   58.641 \\
               MF &    $a_{MV,B,\Sigma}$ & Small &    19.907 &   21.226 \\
               MF &    $a_{MV,B,\Sigma}$ & Large &    52.567 &   70.213 \\
\bottomrule
\end{tabular}

